Temporal Planning via Interval Logic Satisfiability for Autonomous Systems

Many automated planning methods and formulations rely on suitably designed abstractions or simplifications of the constrained dynamics associated with agents to attain computational scalability. We consider formulations of temporal planning where intervals are associated with both action and fluent atoms, and relations between these are given as sentences in Allen's Interval Logic. We propose a notion of planning graphs that can account for complex concurrency relations between actions and fluents as a Constraint Programming (CP) model. We test an implementation of our algorithm on a state-of-the-art framework for CP and compare it with PDDL 2.1 planners that capture plans requiring complex concurrent interactions between agents. We demonstrate our algorithm outperforms existing PDDL 2.1 planners in the case studies. Still, scalability remains challenging when plans must comply with intricate concurrent interactions and the sequencing of actions.

==> temporal_planning.tex <==
\section{Temporal Planning as (Interval Logic) SAT}
\label{sec:TPSAT}

Our notion of \emph{temporal planning} is that of a computational problem where we need to find the definition of a
multi-dimensional \emph{reference signal} $r: \mathbb{T} \to \mathbb{R}^k$ that we require admissible control components
to track, as illustrated by Figure~\ref{fig:planning_control_systems}.
We assume that a feedback control algorithm exists even when $r$ is not smooth, and thus restrict the range of
$r$ to $k$-dimensional vectors of Boolean values.
We further assume that each dimension of our Boolean reference signals is associated with one
$\varphi \in \Atoms{\Sigma}$; these in turn compactly encode either \emph{guard conditions}~\cite{lee:embedded_systems}
defining the modes in which control functions $g(x,r)$ must be at a given point in time, or structural constraints on
$g(x,r)$, when several possible control strategies are available.

\begin{example}
    Predicates $Near(l)$ and $Pointing(l)$ given in Eqs.~\eqref{eq:near_predicate} and~\eqref{eq:pointing_predicate}
    are examples of atomic formulas encoding guard conditions.
    For the example system described in Section~\ref{sec:Example_Model} a reasonable definition for $g(x,r)$ that
    is consistent with $Turn(l)$ would be
    \begin{align*}
        u(k+1) = \begin{cases}
                     \begin{bmatrix}
                          0 & \omega(k) + K_1 e(k) - K_2 T_s \omega(k)T_s
                     \end{bmatrix}^{T} & \mathrm{if}\,h(k, Pointing(l)) = 0 \\
                     \begin{bmatrix}
                          0 & 0
                     \end{bmatrix}^{T} & \mathrm{otherwise}
        \end{cases}
    \end{align*}
    where the entries of the vectors above correspond to $v$ and $\omega$.
\end{example}

Informally, \emph{temporal planning} is the computational problem of finding sets of TQAs $P$ whose properties
express constraints on system inputs $U$ and states $X$ that connect a given initial condition of the system $X_0 \subset X$
with a set of \emph{goal} system states $X_{\star} \subset X$. Additionally, we want $P$ to minimize
a given \emph{objective} function $f$, s.t. $f(P) = c_P$, $c_P \in \mathbb{Q}$.

Let $(\Sigma, V)$ be a given domain theory. An \emph{instance} of a temporal planning problem is given by
the tuple $({\cal F}, {\cal A}, \Sys, X_0, X_{\star})$. $X_0$ and $X_\star$ are as above. ${\cal F}$ and
${\cal A}$ are both finite sets\footnote{
$X_{\varphi} \coloneqq \{ x \in X \,:\, x \models \varphi\}$, similarly for $U_{\alpha}$.
}
where each $X_\varphi \in {\cal F}$ and $X_\varphi \subset X$ (resp. $U_\alpha \in {\cal A}$
and $U_\alpha \subset U$). We will refer to sets $X_\varphi$  and $U_\alpha$ as \emph{fluents} and \emph{actions}, respectively.
We require that for each set $X_\varphi$ (resp. $U_\alpha$) there is a unique atomic formula $\varphi$ (resp. $\alpha$)
in \Fml{\Sigma}{V}, and from now on, we use the latter to refer to fluents and actions. Similarly, $X_0$ and $X_\star$ are
in what follows treated as \emph{conjunctions} of atomic formulae.

$\Sys$ is the set of \emph{system axioms}, each of its elements a universally-quantified formulas using
$(\Sigma, V)$. We distinguish two types of system axioms, i.e. $\Sys$ $=$ $(\Act, \Int)$, which we will refer to as
\emph{action schemas} $\sigma$ and \emph{domain constraints} $\kappa$, respectively. Action schemas are
Interval Logic formulas that describe qualitatively~\cite{kuipers:qsim} the possible state trajectories of a system model
under a particular type of input signals. We describe them in detail below. The domain constraints $\kappa$ encode a relation between
fluents $\varphi$ and $\phi$ in ${\cal F}$ that holds whenever it can be shown that no state $x \in X$ can be both (1)
reachable from $X_0$, and (2) simultaneously satisfy $x \in X_{\varphi}$ and $x \in X_{\phi}$~\cite{gerevini:constraints}. For instance,
atoms $Near(l)$ and $Near(l')$ where $l$ and $l'$ are separated by a distance greater than $d$ would be examples
of such conflicting, or \emph{interfering}, fluents. The domain constraint for this example would be written as
\begin{align*}
    \kappa(l, l') \equiv \big(\Vert q_l - q_{l'} \Vert \geq d_l\big) \rightarrow (\neg Near(l) \lor \neg Near(l'))
\end{align*}
We denote that the interference relation between fluents $\varphi$ and $\phi$ holds by
$\IntRel{\varphi}{\phi}$.

\textbf{Action schemas} are formulas $\sigma(\bar{x}, \bar{I})$ that relate causally and temporally TQAs of fluents and
actions, universally quantified (parameterized) by a vector of variables $\bar{x} \subset V$ of dimension $d$, and a finite set of intervals
$\bar{I} = \{ I_0, \ldots, I_n\}$:
\begin{align}
    \label{def:action_schema}
    \sigma(\bar{x}, \bar{I}) \equiv \forall \bar{x}, \bar{I}\,:\, \alpha(\bar{x})_{I_0} \rightarrow \Gamma(\bar{x}) \land T(\bar{I}) \land A(\bar{x}, \bar{I})
\end{align}
$\Gamma(\bar{x}) \in \Fml{\Sigma}{V}$ is an atemporal formula which restricts the possible vectors $\bar{x}$ action
is supposed to be valid for. We refer to these as \emph{grounding constraints}, and are useful to capture invariant structural
relations between components in a system, such as that between mobile robots and manipulators mounted on each of them.
$A(\bar{x}, \bar{I})$ is a conjunction of fluent TQAs, using each one of the intervals in $\bar{I}$ but $I_0$ which
is reserved for the action TQA, that must follow from an action TQA being in the plan $P$. These
temporally qualified \emph{assertions} identify what fluents or \emph{preconditions} must hold
for the action to be applicable and what other fluents or \emph{effects}\footnote{
We make precise these notions below.
}
become true as a result of applying the action. Finally, $T(\bar{I})$ are \emph{temporal constraints} including both IL atoms $I_{i} \bowtie I_{j}$ where
$\bowtie \in \{ \frown, \supset, = \}$ and \emph{linear constraints} between pairs of bounds of intervals in $\bar{I}$.
For instance, (fixed) action duration is modeled by the atom $r(I_0) - l(I_0) = \delta$, where $\delta > 0$.

%\subsection{Plans}
%\label{Plans}

%A planning problem is thus given by a qualitative system model \Sys, its initial conditions $X_0$, and the goal
%condition $X_{\star}$.

\textbf{Plans} $P$\footnote{
Our notion of plans follows closely~\cite[Chapter 3]{vvaa:plan_reasoning} and borrows key ideas from~\cite{smith:gap}.
}
are taken to be \emph{assumptions} about the future, that is, IL statements about (1) an action $\alpha$ being
applied to the system over some time period $I$, (2) a fluent $\varphi$ truth value being constant through some
time interval $I$, or (3) temporal constraints $I \bowtie I'$ between the intervals featuring in TQAs $\alpha_I$
and $\varphi_{I'}$ put forward as assumptions. We observe that assumptions of types (1) and (2) not only identify
relevant system properties, i.e., actions and fluents, but also, and crucially, time intervals.

We start formalizing the above by making the structure of plans $P$ precise. Initial and goal conditions
are modeled with IL statements by introducing special intervals $I_\prec$ and $I_\succ$, which denote respectively the
time \emph{before} the execution of $P$ commences, and the time \emph{after} the last action in the plan finishes.
For each fluent $\chi_{0} \in X_0$ (resp. $\chi_\star\in X_{\star}$) we define TQAs  $\chi_{0I}$ and $\chi_{\star I}$,
and bind their intervals with temporal constraints to $I_\prec$ and $I_\succ$

\begin{definition}[Plan]
    \label{def:Plans}
    A plan $P$ is given by a tuple $(S, K, C)$ where $S$ is a finite set of fluent TQAs
    $\varphi_{I_1}$, …, $\varphi_{I_n}$, $K$ is a finite set of action TQAs $\alpha_{I_1}$, …,
    $\alpha_{I_m}$, and $C$ is finite set of temporal constraints $\tau_{I,I'}$. The set of
    plan intervals is
    %intervals associated
    %with the assumed system properties in the plan is defined as
    ${\cal I}_P \coloneqq \{I_\prec, I_\succ\} \cup \{ I \,:\, \varphi_I \in S \} \cup  \{ I \,:\, \alpha_I \in K \}$.
    Additionally, (1) for every $\tau_{I,I'} \in C$ it holds that $I, I' \in {\cal I}_P$, (2) for each $\chi \in X_0$
    we have $\chi_{I} \in S$ and $\Meets{I_\prec}{I} \in C$, and (3) for each $\chi \in X_\star$ we have
    $\chi_{I} \in S$ and $\Meets{I}{I_\succ} \in C$.
\end{definition}

For a plan $P$ to solve a planning problem instance, some constraints must be satisfied that restrict the
possible choices of elements in $S$, $K$, and $C$. In this paper, these restrictions follow from two core
STRIPS assumptions: first, that fluents $\varphi$ are \emph{inertial} so their truth value only changes due to an
action being applied, and second, that a singular controlling entity or agent chooses actions in plans. We must separate TQAs asserted by action
schemas $\sigma$ for the first assumption.\footnote{
We drop the variables in schema components signatures to simplify the discussion here. Also, we use $T_\sigma$ and
$A_\sigma$ to refer to the corresponding formulae in~\eqref{def:action_schema}.
} We say that a TQA in the set of assertions of schema $\sigma$, i.e.$\sigma$ $\varphi_I \in A_{\sigma}$,
is an \emph{effect} of action TQA $\alpha_{I_0}$ if and only if we have a temporal constraint
$\alpha_{I_0} \bowtie \alpha_I$ in $T_\sigma$ and
$\bowtie \in \{ \supset, =, \frown \}$. Alternatively, a TQA $\varphi_I$ in $A_\sigma$ is a \emph{precondition} of $\alpha_{I_0}$
if we have $\varphi_{I} \bowtie \alpha_{I_0}$ and $\bowtie \in \{\supset, \frown \}$. We now have in place all the elements to define when
plans $P$ are admissible as solutions of planning problem instances%, or \emph{valid}

\begin{definition}[Valid Plans]
    \label{def:Valid_Plans}
Let $P=(S, K, C)$ be a plan.
We say plan $P$ is \emph{valid} iff the following holds: (1) for every $\varphi_I$ in $S$ such that $\Before{I_\prec}{I}$
there must be a TQA $\alpha_{I'}$ in $K$ such that $\varphi_I$ is an effect of
$\alpha_{I'}$, (2) for every $\alpha_I \in K$ with schema $\sigma$ we have TQAs and temporal constraints in $S$ and $C$ matching
those in $A_\sigma$ and $T_{\sigma}$, (3) for every pair of TQAs $\varphi_I$ and $\phi_{I'}$ in $S$ for which
$\IntRel{\varphi}{\phi}$ holds, we have that $I \mid\mid I'  \in C$, and (4) ${\cal I}_P, h \models S \land K \land C$
    for some $h$.
\end{definition}


\emph{Optimal plans} w.r.t. an objective function $f$ are thus defined as the set of \emph{valid} plans $P^\star \in \Pi^{\star}$
so that for every other valid plan $P'$ then $f(P^\star) \leq f(P')$. Classical cost functions in Operations Research~\cite{hooker:10:integrated}
such as \emph{makespan}, \emph{sum of costs} and \emph{tardiness} can be all easily formulated.


==> timing_diagrams.tex <==
\section{Datelines for Framing Temporal Plans}
\label{section:datelines}

A key difficulty found by previous formulations of constraint-based interval planning~\cite{smith:gap} is that
of identifying and managing plan  intervals ${\cal I}_P$.
To overcome this challenge, we propose a novel hierarchical,
compositional temporal structure to ``frame'' TQAs in plans, illustrated by
Figure~\ref{fig:Dateline_Illustration}. We start by

We exploit this result to define plan intervals in this way

In words, ${\cal I}_{P,N}$ is a two-tiered temporal structure that provides a ground set of intervals to define
\emph{multiple} TQAs using fluents and complex, non-atomic IL sentences. Searching for a plan $P$ thus becomes the problem of choosing how
to ``bundle'' together the elements of ${\cal I}_{P,N}$ in a way consistent with Definition~\ref{def:Valid_Plans}.
The value $N$
for which we can find a plan $P$ that satisfies Definition~\ref{def:Valid_Plans} depends on how many times a fluent
needs to change its truth value, how many instances of an action are necessary, and how many actions are required to
be sequenced to achieve a sub-goal, and how concurrent TQAs interact during plans.

